Mathematics Is Imprecise

We commonly think of mathematics as bringing precision to application domains, but its relationship with computer science is more complex. This experience report on the use of Racket and Haskell to teach a required first university CS course to students with very good mathematical skills focusses on the ways that programming forces one to get the details right, with consequent benefits in the mathematical domain. Conversely, imprecision in mathematical abstractions and notation can work to the benefit of beginning programmers, if handled carefully.

==> eptcsdata.tex <==
\providecommand{\firstpage}{40}
\providecommand{\publicationstatus}{M. Moraz\'an and P. Achten (Eds.): Trends in Functional \\ Programming in Education 2012 (TFPIE 2012).\\
EPTCS 106, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.106.3}{10.4204/EPTCS.106.3}}

